A General Theory of Propositional Modal Bundled Modalities

In studies of bundled modalities, we encode a complex conceptual notion into the semantics of a single modal operator and study its logic. Although there is already a substantial body of work on various concrete bundled operators, we still lack a general understanding of them. In this paper, we provide a general theory of the expressivity and axiomatization of bundled modalities. We offer a uniform way to define bisimulations for arbitrary bundled modalities and justify our definition by the corresponding Hennessy-Milner property. We also define a special class of bundled modalities called positive-negative-independent bundles. This class of bundles, together with their duals, cover most bundled modalities studied in the literature, and their axiomatizations can be done with the help of a more abstract notion of convex neighborhood semantics and corresponding representation results. As case studies, we axiomatize the "someone knows" bundle $\bigvee_{a \in A} \Box_a \phi$ over $S5$-models, the ``disagreement within group'' bundle $\bigvee_{a, b \in A} \Box_a \phi \wedge \Box_b \neg \phi$ over $KD45$-models, and the "belief without knowledge" bundle $B \phi \wedge \neg K \phi$ over $S4.2$-models.

==> eptcsdata.tex <==
\providecommand{\firstpage}{299}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.17}{10.4204/EPTCS.447.17}}

